Detection of the Keplerian decline in the Milky Way rotation curve

Our position inside the Galactic disc had prevented us from establishing an accurate rotation curve, until the advent of Gaia, whose third data release (Gaia DR3) made it possible to specify it up to twice the optical radius. We aim to establish a new rotation curve of the Galaxy from the Gaia DR3, by drastically reducing uncertainties and systematics, and with the goal to provide a new estimate of the mass of the Galaxy. We have compared different estimates, established a robust assessment of the systematic uncertainties, and addressed differences in methodologies, particularly regarding distance estimates. This results in a sharply decreasing rotation curve for the Milky Way, the decrease in velocity between 19.5 and 26.5 kpc is approximately 30 km s$^{-1}$. We have identified, for the first time, a Keplerian decline of the rotation curve, starting at $\sim$ 19 kpc and up to $\sim$ 26.5 kpc from the Galaxy center, while a flat rotation curve is rejected with a significance of 3$\sigma$. The total mass is revised downwards to $2.06^{+0.24}_{-0.13}\times 10^{11}\ M_{\odot}$, in agreement with an absence of significant mass increase at radii larger than 19 kpc. The upper limit of the total mass was evaluated by considering the upper values of velocity measurements, which leads to a strict, unsurpassable, limit of $5.4\times 10^{11}\ M_{\odot}$.

==> mass.tex <==
\begin{table*}[h]
    \centering
    \caption{Estimated MW dynamical mass and associated Einasto profile parameters for RC of this work (TW) and \citet[][O23]{ou2023}. }
    \begin{tabular}{lccccccccc}
    \hline \hline
    Baryon model & $M_\mathrm{bar}$ & \multicolumn{2}{c}{$M_\mathrm{dyn}$} & \multicolumn{2}{c}{$M_\mathrm{0}$} & \multicolumn{2}{c}{h} & \multicolumn{2}{c}{n} \\
    & [$10^{11} M_{\sun}]$ & \multicolumn{2}{c}{[$10^{11} M_{\sun}$]} & \multicolumn{2}{c}{[$10^{11} M_{\sun}$]} & \multicolumn{2}{c}{[kpc]} & \multicolumn{2}{c}{} \\
    % & &\multicolumn{4}{l}{This work with systematics}  & \multicolumn{4}{l}{\citet{ou2023} with systematics}  \\
    %\hline
    &&TW&O23&TW&O23&TW&O23&TW&O23\\
    \hline
    B2 & 0.616 & $2.05^{+0.08}_{-0.06}$ & $2.19^{+0.17}_{-0.12}$ & $3.72^{+0.45}_{-0.70}$  & $1.23^{+0.63}_{-0.58}$ & $11.41^{+1.15}_{-1.62}$ & $5.5^{+1.46}_{-1.56}$ & $0.43^{+0.12}_{-0.09}$ & $0.87^{+0.20}_{-0.15}$\\
    E dJ & 0.607 & $1.97^{+0.09}_{-0.06}$ & $2.07^{+0.15}_{-0.11}$ & $3.72^{+0.36}_{-0.63}$  & $1.82^{+0.64}_{-0.72}$ & $12.30^{+1.10}_{-1.63}$ & $7.3^{+1.46}_{-1.74}$ & $0.40^{+0.13}_{-0.09}$ & $0.73^{+0.18}_{-0.14}$ \\
    E J & 0.603 & $1.97^{+0.09}_{-0.06}$ & $2.08^{+0.16}_{-0.11}$ & $3.72^{+0.36}_{-0.70}$  & $1.70^{+0.65}_{-0.72}$ & $12.21^{+1.12}_{-1.68}$ & $7.03^{+1.49}_{-1.79}$ & $0.40^{+0.13}_{-0.09}$ & $0.76^{+0.19}_{-0.14}$\\
    E CM & 0.589 & $1.97^{+0.09}_{-0.06}$ & $2.10^{+0.17}_{-0.12}$ & $3.55^{+0.43}_{-0.73}$  & $1.26^{+0.69}_{-0.61}$ & $11.63^{+1.20}_{-1.77}$ & $5.81^{+1.58}_{-1.71}$ & $0.43^{+0.14}_{-0.10}$ & $0.85^{+0.21}_{-0.16}$ \\
    G dJ & 0.575 & $1.98^{+0.09}_{-0.07}$ & $2.14^{+0.17}_{-0.12}$ & $3.47^{+0.51}_{-0.78}$  & $1.02^{+0.64}_{-0.52}$ & $11.34^{+1.28}_{-1.86}$ & $4.99^{+1.52}_{-1.54}$ & $0.45^{+0.15}_{-0.10}$ & $0.94^{+0.21}_{-0.17}$ \\
    G J  & 0.571 & $1.98^{+0.09}_{-0.06}$ & $2.15^{+0.19}_{-0.13}$ & $3.39^{+0.50}_{-0.76}$  & $0.89^{+0.62}_{-0.51}$ & $11.29^{+1.26}_{-1.82}$ & $4.72^{+1.60}_{-1.64}$ & $0.45^{+0.14}_{-0.10}$ & $0.97^{+0.24}_{-0.18}$ \\
    G CM & 0.557 & $1.99^{+0.10}_{-0.07}$ & $2.16^{+0.18}_{-0.13}$ & $3.31^{+0.58}_{-0.91}$  & $0.64^{+0.56}_{-0.38}$ & $10.63^{+1.40}_{-2.01}$ & $3.85^{+1.52}_{-1.35}$ & $0.49^{+0.16}_{-0.11}$ & $1.06^{+0.23}_{-0.19}$ \\
     \hline
     Average & & $1.99^{+0.09}_{-0.06}$ & $2.13^{+0.17}_{-0.12}$\\
    \hline
    %\multicolumn{8}{l}{$^a$ \yj{Dynamical mass $M_\mathrm{dyn}$ equals to the sum of baryon mass $M_\mathrm{bar}$ and DM virial mass $M_\mathrm{vir}.}}
    \end{tabular}
    \label{tab:mass}
\end{table*}

==> para_bulge.tex <==
\begin{table}
\centering
\caption{Parameters of bulge, see more details in Section~\ref{sec:bary}}
\begin{tabular}{l l l l}
    \hline \hline
    Parameter & bulge E & bulge G & bulge B2 \\
    \hline
    $M_{\mathbf{bulge}} (10^{10} M_{\odot})$ & 1.962 & 1.639  & 1.550 \\
    $x_\mathrm{b}(\mathrm{kpc})$    &0.899&1.239& 0.700$^a$\\
    $y_\mathrm{b}(\mathrm{kpc})$    &0.386&0.609& ----\\
    $z_\mathrm{b}(\mathrm{kpc})$    &0.250&0.438& ----\\
    \hline
    \multicolumn{4}{l}{$^a$ Value of $r_b$ in Eq.~\ref{eq:hernq}}
    \end{tabular}
\label{tab:bulge}
\end{table}

==> para_disk.tex <==
\begin{table}
\centering
\caption{Parameters of disk, see more details in Section~\ref{sec:bary} }
\begin{tabular}{l l l l l}
    \hline \hline
    Parameter & disk CM  & disk J & disk dJ & disk B2\\
    \hline
    $M_{\mathbf{thin}} (10^{10} M_{\odot})$ & 3.11&3.17&3.33 & 3.65\\
    $M_{\mathbf{thick}} (10^{10} M_{\odot})$ &0.82&0.90&0.78&----\\
    $L_{\mathbf{thin}} (\mathrm{kpc})$ &2.75&2.60&2.60&2.35\\
    $L_{\mathbf{thick}} (\mathrm{kpc})$ &4.10&3.60&4.10&----\\
    $H_{\mathbf{thin}} (\mathrm{kpc})$ &0.25&0.30&0.25&0.14\\
    $H_{\mathbf{thick}} (\mathrm{kpc})$ &0.75&0.90&0.75&----\\
    \hline 
\end{tabular}
\label{tab:disk}
\end{table}

==> rc_mw_z3.tex <==
\begin{table}
\centering
\caption{Measurements of the Circular Velocity of the Milky Way.}
\begin{tabular}{ccc}
\hline \hline
$R$ [kpc] & $V_c$ [km s$^{-1}$] & $\sigma_{V_c}$ [km s$^{-1}$]\\
\hline
9.5 & 221.75 & 3.17 \\
10.5 & 223.32 & 3.02 \\
11.5 & 220.72 & 3.47 \\
12.5 & 222.92 & 3.19 \\
13.5 & 224.16 & 3.48 \\
14.5 & 221.60 & 4.20 \\
15.5 & 218.79 & 4.75 \\
16.5 & 216.38 & 4.96 \\
17.5 & 213.48 & 6.13 \\
18.5 & 209.17 & 4.42 \\
19.5 & 206.25 & 4.63 \\
20.5 & 202.54 & 4.40 \\
21.5 & 197.56 & 4.62 \\
22.5 & 197.00 & 3.81 \\
23.5 & 191.62 & 12.95 \\
24.5 & 187.12 & 8.06 \\
25.5 & 181.44 & 19.58 \\
26.5 & 175.68 & 24.68 \\
\hline
\end{tabular}
\label{tab:rc_z3}
\end{table}

